A Unified Linear Programming Framework for Offline Reward Learning from Human Demonstrations and Feedback

Inverse Reinforcement Learning (IRL) and Reinforcement Learning from Human Feedback (RLHF) are pivotal methodologies in reward learning, which involve inferring and shaping the underlying reward function of sequential decision-making problems based on observed human demonstrations and feedback. Most prior work in reward learning has relied on prior knowledge or assumptions about decision or preference models, potentially leading to robustness issues. In response, this paper introduces a novel linear programming (LP) framework tailored for offline reward learning. Utilizing pre-collected trajectories without online exploration, this framework estimates a feasible reward set from the primal-dual optimality conditions of a suitably designed LP, and offers an optimality guarantee with provable sample efficiency. Our LP framework also enables aligning the reward functions with human feedback, such as pairwise trajectory comparison data, while maintaining computational tractability and sample efficiency. We demonstrate that our framework potentially achieves better performance compared to the conventional maximum likelihood estimation (MLE) approach through analytical examples and numerical experiments.

==> sections/experiment_arXiv.tex <==


\section{Numerical Experiments}\label{sec:experiment}

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=.48\textwidth]{figures/Figure_1.pdf}
\hfill
\includegraphics[width=.48\textwidth]{figures/Figure_2.pdf}
\caption{$\mathcal{L}^1$ error in the optimal occupancy measure under an estimated reward function. Left: Offline IRL algorithms; Right: Offline RLHF algorithms.}
\label{fig:irl}
\end{center}
\vskip -0.2in
\end{figure*}

In this section, we demonstrate the performance of our LP algorithms through numerical experiments, comparing them to MLE algorithms in the literature.
We consider an MDP with $|S|=10$, $|A|=2$, and $\gamma=0.95$. In each experimental run, $P$ and $\mu_0$ are randomly selected.
To introduce additional complexity to the problem, we have set the true rewards to have similar values: $r_{\text{true}}(s, a_1) = 1.0$ and $r_{\text{true}}(s, a_2) = 0.9$ for all states $s\in S$.
The performance of each algorithm is assessed by measuring the proximity of an optimal occupancy measure under the true reward $r_\text{true}$ and the estimated reward function $\hat{r}$.
Specifically, we report $\Vert d^*(r_\text{true}) - d^*(\hat{r})\Vert_1$, which represents the $\mathcal{L}^1$ error between the optimal occupancy measures under $r_\text{true}$ and $\hat{r}$.
In each experiment, we sample $N$ trajectories with a horizon of $H=20$ according to $\pi_e$ in IRL, and $\mu_\text{HF}$ in RLHF.
For each sample size $N$, we conducted 200 experiments and reported the mean and standard deviation of the error.
See Appendix~\ref{app:experiment} for detailed parameters and algorithms used in the experiments.

\paragraph{Offline IRL.}
The left side of Figure~\ref{fig:irl} compares the errors associated with each IRL algorithm. The results indicate that our LP-based algorithms generally outperform the bi-level optimization-based MLE algorithm~\cite{zeng2023understanding}, demonstrating that LP is more sample-efficient in addressing ambiguity in the dynamics and the expert policy.
The solution set with a smaller relaxation level $\epsilon_g = 0.001/\sqrt{N}$ (LP-IRL-2) exhibits better performance than that with a greater relaxation level $\epsilon_g = 0.01/\sqrt{N}$ (LP-IRL-1).
This is consistent with the optimality-feasibility trade-off discussed in Section~\ref{sec:IRLoptimality}.
Additionally, the integration of IRL and RLHF data leads to improved performance, as predicted. The use of continuous feedback (LP-IRL-C) is even more effective than discrete feedback (LP-IRL-D) by facilitating stricter constraints.

\paragraph{Offline RLHF.}
In numerical experiments for offline RLHF, the human feedback data is generated following the greedy model.
The right side of Figure~\ref{fig:irl} compares the reward function obtained from LP~\eqref{eq:RLHFset} and the pessimistic MLE algorithm proposed by~\cite{zhu2023principled} under the BTL model.
In the LP algorithm, the error decreases rapidly as the number of samples increases, whereas the error in the MLE algorithm decreases more slowly.
This result is consistent with the discussion in Appendix~\ref{app:mle}, suggesting that the MLE algorithm might be inefficient or even fail if the human evaluator deviates from the assumed model, whereas LP does not.



==> sections/introduction_arXiv.tex <==

\section{Introduction}
Reward learning involves inferring and shaping the underlying reward function from observed human demonstrations and feedback.
Inverse reinforcement learning (IRL) and reinforcement learning from human feedback (RLHF, also known as preference-based reinforcement learning) are key methodologies in reward learning, applied in various sequential decision-making tasks such as games~\cite{macglashan2017interactive, christiano2017deep, ibarz2018reward}, robotics~\cite{finn2016guided, brown2019extrapolating, shin2023benchmarks}, and language models~\cite{ziegler2019fine, stiennon2020learning, wu2021recursively, ouyang2022training, liu2023chain}.
Particularly in the recent drastic development of large language models (LLMs), RLHF has played a crucial role in fine-tuning models to better align with human preferences~\cite{ouyang2022training}.
However, despite the notable empirical success of these algorithms, a significant gap remains in the theoretical analysis of IRL and RLHF, limiting us to guarantee their reliability.
This work aims to bridge this gap by proposing a novel theoretical framework for offline IRL and RLHF.

IRL aims to infer a reward function that aligns with an expert behavior from demonstrations~\cite{ng2000algorithms, abbeel2004apprenticeship}.
Typical IRL algorithms employ a bi-level optimization framework within the context of maximum likelihood estimation (MLE).
In this framework, the inner optimization evaluates the policy based on the current reward parameters, while the outer optimization updates these parameters to better match observed expert behavior.
These algorithms have been extensively explored in the literature~\cite{ziebart2008maximum, wulfmeier2015maximum, zhou2017infinite, zeng2022structural, zeng2023understanding}, and their convergence is studied in both online settings~\cite{zeng2022structural} and offline settings~\cite{zeng2023understanding}.

Building upon IRL, RLHF recovers a reward function from human feedback data, which is commonly given by pairwise or $K$-wise trajectory comparisons. 
Despite growing interest in RLHF, only a few algorithms provide optimality guarantees with sample complexity bound.
Most existing approaches adopt an MLE framework, assuming that human evaluators follow a presupposed preference model, such as the Bradley-Terry-Luce (BTL) model.
The reward parameters are then fine-tuned to maximize the log-likelihood of the collected offline preference data~\cite{christiano2017deep}.
Recently, \cite{zhu2023principled, zhan2023provable, li2023reinforcement} have proposed offline RLHF algorithms with optimality guarantees by adopting a pessimistic mechanism from offline reinforcement learning (RL) theory.
\cite{park2024principled} further suggested a personalized setting that learns multiple reward models for heterogeneous preferences.


While the MLE-based approach offers a solid theoretical framework for both IRL and RLHF, it comes with unavoidable limitations.
Particularly in IRL, bi-level optimization algorithms face computational challenges due to their nested-loop structures.
In addition, MLE-based algorithms rely on a specific decision-making or preference model they employ.
For example, the IRL algorithm proposed by~\cite{zeng2022structural} learns the reward function that aligns with an expert policy, which is assumed to be an optimal softmax policy.
Furthermore, RLHF algorithms (e.g. \cite{zhu2023principled, zhan2023provable}) assume a preference model for human evaluator, which might not fully capture the complex and diverse nature of real-world human preferences.
Consequently, their optimality guarantees might be compromised if there exists a  mismatch between actual human preferences and the model in use.

In response to these challenges inherent in MLE frameworks, recent research has shifted focus from estimating a single reward function (under a presupposed model) to recovering a \emph{feasible reward set}, a set of rewards where the expert policy is (near) optimal.
Notably, \cite{metelli2021provably, metelli2023towards} estimated the feasible reward set from finite-horizon Bellman equations and provided sample complexity bounds associated with estimation errors.
However, their algorithm requires a generative model of state transition probabilities.
\cite{lindner2022active} mitigated this requirement by adopting an efficient exploration policy for sampling trajectories, though it remains in an online setting.
More recently, and concurrent with our work, \cite{zhao2023inverse} introduced the first offline algorithm with a theoretical guarantee.
They introduce a pessimistic mechanism to address the issue of non-uniform data coverage, penalizing state-action pairs with low visitation frequency. 
Nevertheless, these penalty functions are nonlinear and non-convex, resulting in a non-convex reward set.
This could limit flexibility for applications, especially when selecting a specific reward function within the set.

In line with this evolving perspective, we aim to obtain a \emph{convex estimate} of a feasible reward set in an offline setting.
To achieve this, we leverage recent advancements in the Linear Programming (LP) framework within the domain of offline RL.
A fundamental challenge in offline RL is the non-uniform coverage of offline data ~\cite{fujimoto2019off, kumar2020conservative}.
To address this issue, recent algorithms have employed a pessimistic mechanism that conservatively selects the value function or model within an uncertainty set~\cite{liu2020provably, jin2021pessimism, rashidinejad2021bridging, xie2021bellman,uehara2021pessimistic, chen2022offline}.
However, these pessimistic approaches often introduce non-convex optimization problems, which can be intractable.
In the latest research, a series of works~\cite{zhan2022offline, rashidinejad2022optimal, ozdaglar2023revisiting} have introduced LP-based methods that relax data coverage assumptions and provide tractable algorithms suitable for function approximation by introducing convex formulations.

Given the success of LP-based approaches in offline RL, investigating how it could address non-convexity and non-uniform data coverage issues in offline IRL presents a promising research direction.
One notable advantage of LP is its flexibility in addressing intrinsic challenges in reward learning, such as avoiding undesirable degenerate solutions like $r=\mathbf{0}$.
We demonstrate that a polyhedral estimate of the feasible reward set, provided by LP, offers efficient ways to identify a non-degenerate reward function.
For example, it allows to select a reward function that maximizes the reward gap between the expert policy and suboptimal policies (e.g., uniform policy) over the solution set.
We also highlight LP's suitability for function approximation, primarily due to its linear structure, which can further reduce the solution set and computational complexity.
Furthermore, the LP framework enables the integration of extra information.
As a notable example, we show that RLHF data can be incorporated by simply adding linear constraints, maintaining computational tractability and sample efficiency.

Our main contributions can be summarized as follows:
\begin{itemize}
    \item We present an LP formulation for offline IRL that directly estimates the feasible reward set by the primal-dual optimality conditions in an empirical LP formulation of Markov decision process (MDP) (Section~\ref{sec:IRLformulation}).
    \item In Theorem~\ref{thm:optimality}, the optimality of the estimated reward set is provided such that any reward function within this set ensures the expert policy is $\tilde{O}(\sqrt{|S||A|/N})$-suboptimal, under appropriate data coverage assumption.
    \item In offline RLHF, we align reward functions with pairwise trajectory comparison data using linear constraints (Section~\ref{sec:RLHFformulation}).
    In Theorem~\ref{thm:rlhf}, we provide the generalization guarantee of the estimated reward function for unseen trajectory pairs.
    \item We address the potential degeneracy issue in reward learning (Section~\ref{sec:IRLdegeneracy}) and propose a unified framework that effectively combine IRL and RLHF to mitigate the degeneracy (Section~\ref{sec:integration}).
    \item The proposed LP algorithm and the MLE algorithms in the literature are compared through numerical experiments (Section~\ref{sec:experiment}).
    We also provide an analytical example in offline RLHF, where MLE algorithm fails, while our LP approach succeeds to identify the optimal policy (Appendix~\ref{app:mle})
\end{itemize}
Additional related literature is discussed in Appendix~\ref{app:relatedwork}.

==> sections/section2_arXiv.tex <==


\section{Preliminaries}


\subsection{Markov Decision Process (MDP)}
We first revisit the standard notations for a tabular infinite-horizon discounted Markov decision process (MDP).
An MDP $\mathcal{M}$ is represented as a tuple $\mathcal{M} = (S, A, P, \gamma, \mu_0, r)$, where $S$ and $A$ represent finite state and action spaces, $P: (S, A) \mapsto \Delta(S)$ denotes the transition probability function, $\gamma \in (0, 1)$ represents the discount factor, and $\mu_0 \in \Delta(S) $ is the initial state distribution.
The reward function $r(s,a): S \times A \mapsto [-1, 1]$ indicates the reward received for taking the action $a$ in state $s$.

The primary objective in MDP is to identify a stochastic policy $\pi:S \mapsto \Delta(A)$ that maximizes the expected cumulative reward: $\mathbb{E}^\pi [\sum_{h=0}^\infty \gamma^h r(s_h, a_h) | s_0 \sim \mu_0]$.
We define $v^\pi(s)$ as the expected total discounted reward received when initiating from state $s$ and following $\pi$, such that $v^\pi(s) := \mathbb{E}^\pi\left[\sum_{h=0}^\infty \gamma^h r(s_h, a_h) \mid s_0 = s\right]$.
Then, the optimal policy $\pi^*$ maximizing the expected reward and its corresponding value function $v^* := v^{\pi^*}$ are related by the Bellman equation
\begin{equation}
v^*(s) = \max_{a \in A} \left\{ r(s,a) + \gamma \sum_{s' \in S} P(s' | s, a) v^*(s') \right\},
\end{equation}
which holds for any $s \in S$.
It is well-established that $v^*$ can be determined by solving the following linear programming (LP) as outlined in~\cite{puterman2014markov}:
\begin{equation}
\min_{v \in \mathbb{R}^{|S|}} \;  (1-\gamma)\mu_0^\top v \quad \text{s.t.} \quad M^\top v - r \geq 0.
\end{equation}
The matrix $M \in \mathbb{R}^{|S|^2|A|}$ is defined as  $M(s', (s,a)) := \mathbf{1}_{\{s' = s\}} - \gamma P(s' | s,a)$, where $\mathbf{1}_{\{s' = s\}}$ denotes the indicator function for the case $\{s'=s\}$.
Throughout the paper, we treat the above LP as the primal LP, and $v$ as the primal optimization variable.
Then, the dual LP is expressed as
\begin{equation}
\max_{d\in \mathbb{R}^{|S||A|}} \;  r^\top d \quad \text{s.t.} \quad  M d = (1-\gamma)\mu_0 , \quad  d \geq 0.
\end{equation}
The dual variable $d$, often interpreted as an \emph{occupancy measure} or a discounted state-action visitation frequency in RL literature, is related to a policy $\pi$ by
\begin{equation}
d^\pi (s, a) = (1-\gamma) \sum_{h=0}^\infty \gamma^h P^\pi_{\mu_0} (s_h = s, a_h = a).
\end{equation}
Here, $P^\pi_{\mu_0} (s_h = s, a_h = a)$ represents the probability of $(s_h, a_h) = (s, a)$, given $s_0 \sim \mu_0$ and $a_{h'} \sim \pi(s_{h'})$ for all $h' \geq 0$.
The dependence on $\gamma$ and $\mu_0$ is omitted in the notation $d^\pi$ for simplicity.
A more detailed relationship between $\pi$ and $d^\pi$ can be found in~\cite{puterman2014markov}.

 

\subsection{Offline IRL: Learning from Expert Trajectories}
While RL learns a policy to maximize rewards in a given environment, IRL aims to infer the underlying reward function that drives observed behavior.
In the standard IRL setting, a single expert agent collects trajectory (roll-out) samples, and the reward function is recovered from these samples.
We denote the true expert policy and corresponding occupancy measure as $\pi_e$ and $d_e$, respectively, where $d_e$ is defined as $d_e := d^{\pi_e}$.
Our objective is to learn a reward function $r$ such that the occupancy measure $d_e$ is (near) optimal, utilizing the offline dataset gathered from the expert policy $\pi_e$. 

In offline setting, the true values of the expert policy $\pi_e$ and the transition probability $P$ are unknown.
Instead, we have access to a static, pre-collected dataset $\mathcal{D}_\text{IRL}$ composed of $N$ independent and identically distributed (i.i.d.) trajectory samples:
\begin{equation}
\mathcal{D}_\text{IRL} = \{\tau^n = (s_0^{n}, a_0^{n}, s_1^{n}, \ldots, s_{H-1}^{n}, a_{H-1}^{n}, s_H^{n} )\}_{n=1}^N.
\end{equation}
Note that the sampling distribution is fully determined by $\mu_0$, $P$, and $\pi_e$.
Let $N_h(s,a)$ and $N_h(s,a,s')$ be the counts of $n$ satisfying $(s_h^n, a_h^n) = (s,a)$ and $(s_h^n, a_h^n, s_{h+1}^n) = (s, a, s')$ in the dataset, respectively.
Using these counts, we estimate the occupancy measure $d_e$ as follows:
\begin{equation}
    \hat{d}_e(s,a) =  (1-\gamma) \frac{1}{N} \sum_{h=0}^{H-1} \gamma^h N_h (s,a) \quad \forall (s,a) \in S \times A.
\end{equation}
Using this empirical estimate $\hat{d}_e$, we aim to develop an LP formulation that identifies a reward function which ensures the optimality of $d_e$ with an acceptable level of error.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Offline RLHF: Learning from Pairwise Trajectory Comparisons}\label{sec:formulation:feedback}
We extend our LP framework to address the offline RLHF problem. Our primary objective is to derive a reward function that is aligned with pairwise trajectory comparison data, provided by human evaluators.
We denote each comparison query as $q_n$, with the index $n$ ranging from 1 to $N_q$.
Each query comprises a pair of trajectories, such that $\tau^{n, 1} = (s_0^{n, 1}, a_0^{n, 1}, \ldots, s_{H-1}^{n, 1}, a_{H-1}^{n, 1}, s_H^{n, 1})$ and $\tau^{n, 2} = (s_0^{n, 2}, a_0^{n, 2}, \ldots, s_{H-1}^{n, 2}, a_{H-1}^{n, 2}, s_H^{n, 2})$.
We assume $\tau^{n, 1}$ and $\tau^{n, 2}$ are sampled i.i.d. according to the sampling distribution $\mu_\text{HF}$.
In each query, a human evaluator is presented with both trajectories and asked to select the one they prefer. 
We denote the event where trajectory $\tau^{n,1}$ is preferred over $\tau^{n,2}$ by the variable $y^n = 1$, and conversely, $y^n = 2$ indicates the event where $\tau^{n,2}$ is favored over $\tau^{n,1}$.
The human feedback dataset is then represented by $\mathcal{D}_\text{HF} = \{ (\tau^{n, 1}, \tau^{n, 2}, y^n) \}_{n=1}^{N_q}$.

Given the dataset $\mathcal{D}_\text{HF}$, we design an LP formulation to identify a reward function $r$ that aligns well with $\mathcal{D}_\text{HF}$.
Notably, this LP approach is purely data-driven, relying solely on the observed comparisons without assuming any specific preference model associated with human evaluators.
This aspect distinguishes it from previous MLE algorithms for offline RLHF.
The detailed comparison will be elaborated in a later section of the paper.

==> sections/section3_arXiv.tex <==
\section{Offline Inverse Reinforcement Learning}
\subsection{LP Formulation of Offline IRL}\label{sec:IRLformulation}
Recall the dual LP formulation of MDP presented in the previous section:
\begin{equation}\label{eq:dual}
\begin{split}
\max_{d \in \mathbb{R}^{|S||A|}} \;  r^\top d \quad \text{s.t.} \quad  M d = (1-\gamma)\mu_0 , \quad  d \geq 0.
\end{split}
\end{equation}
IRL aims to find a feasible reward function $r$ such that the expert occupancy measure $d_e$ is an optimal solution to the above dual LP.
As the feasible reward function is not unique, we define the feasible reward set as follows:
\begin{equation}
    \mathcal{R} = \{r \in [-1, 1]^{|S||A|} \mid d_e \text{ is optimal to \eqref{eq:dual}}\}
\end{equation}
In the offline setting, recovering the ground-truth $\mathcal{R}$ is challenging since we only have access to the empirical estimate of $d_e$ and the transition matrix $P$.
Consequently, our goal is to recover an estimate of $\mathcal{R}$ in which $d_e$ is a near-optimal solution to~\eqref{eq:dual} for any $r$ in this estimated set.


\paragraph{Marginal importance sampling.}
The primary challenge in offline RL and IRL is the non-uniform coverage of the offline dataset.
To address this issue, we adopt the marginal importance sampling (MIS) framework in the literature~\cite{nachum2019algaedice, lee2021optidice}, which considers the scaled version of LP.
First, we define the optimization variable $w_d \in \mathbb{R}^{|S||A|}$ as
\begin{equation}\label{eq:w}
w _d(s,a) := \begin{cases}\frac{d(s,a)}{d_e(s,a)} \quad &\text{if} \quad d_e(s,a) > 0, \\ 0 \quad &\text{if} \quad d_e(s,a) = 0. \end{cases}
\end{equation}
$w_d$ is a scaled dual variable, which represents the ratio between the target $d$ and the expert $d_e$.
The expert optimization variable is denoted by $w_e := w_{d_e}$, which satisfies $w_e (s,a) = \mathbf{1}_{\{d_e(s,a) > 0\}}$ for all $(s, a) \in S \times A$ by the definition of $w_d$.
Note that our algorithm will not require information about which state-action pairs have zero visitation frequency under $\pi_e$ (i.e., $d_e(s,a)=0$), since it will automatically set the reward to zero, i.e. $r(s,a)=0$, if $\hat{d}_e(s,a)=0$.
 
Next, we define $u\in \mathbb{R}^{|S||A|}$ and $K \in \mathbb{R}^{|S|^2|A|}$ as
\begin{equation}
\begin{split}
u(s,a) & := r(s,a) d_e (s,a),\\
K(s', (s,a)) & := d_e (s,a) \mathbf{1}_{\{s= s'\}} - \gamma d'_{e} (s, a, s'),
\end{split}
\end{equation}
where $d'_e (s, a, s') := d_e(s,a) P(s'|s,a)$ for any $(s,a,s')$.
In this MIS framework, $u$ and $K$ correspond to $r$ and $P$, respectively.
The following lemma shows this relationship clearly (see Lemma 1 in~\cite{ozdaglar2023revisiting} for the proof).
\begin{lemma}\label{lem:substitution}
 $r^\top d = u^\top w_d$ and $Md = Kw_d$ hold for any $d\in \mathbb{R}^{|S||A|}$.
\end{lemma}



\paragraph{Empirical LP formulation.}
By Lemma~\ref{lem:substitution}, the dual LP can be written with $u$, $w$, and $K$ as follows:
\begin{equation}
\max_{w \in \mathbb{R}^{|S||A|}} \; u^\top w \quad \text{s.t.} \quad  K w =  (1-\gamma)\mu_0,\quad w \geq 0.
\end{equation}
We omit the subscript $d$ in $w_d$ for ease of notation.
In the above LP formulation, our objective is to identify the set of $u$ for which $w_e$ is optimal.
However, in the offline setting, the true values of $K$ and $d_e$ remain unknown.
Therefore, our goal shifts towards constructing an empirical version of this LP.
We first define the empirical estimate of $u$ as $u_\mathcal{D}(s,a) := r(s,a) \hat{d}_e(s,a)$ for all $(s,a) \in S \times A$, and replace the objective function $u^\top w$ with $u_\mathcal{D}^\top w$.
Next, we introduce $K_\mathcal{D} \in \mathbb{R}^{|S|^2|A|}$, an empirical estimate of $K$, defined as:
\begin{equation}
K_\mathcal{D}(s', (s,a)) := \hat{d}_e(s,a) \mathbf{1}_{\{s = s'\}} - \gamma \hat{d}'_e(s, a, s'),
\end{equation}
where for any $(s,a, s') \in S \times A \times S$,
\begin{equation}
    \hat{d}'_e(s,a, s') := (1-\gamma) \frac{1}{N} \sum_{h=0}^{H-1} \gamma^h N_h(s,a, s').
\end{equation}
However, directly substituting the empirical estimate $K_\mathcal{D}$ for $K$ in the equality constraint $Kw = (1-\gamma)\mu_0$ can be problematic, as it may cause the target variable $w_e$ being infeasible.
 Therefore, we opt to relax the equality constraint to an inequality constraint.

Let $X = [ x_1, \cdots, x_{N_X} ] \in \mathbb{R}^{|S|\times N_x} $ be a coefficient matrix for the relaxation, where $\Vert x_i \Vert_\infty \leq 1 $ for all $i \in \{1, \ldots, N_x\}$.
Let $\epsilon_x \in \mathbb{R}^{N_x}$ be a parameter that controls the level of relaxation.
Then, we replace the equality constraint $Kw = (1-\gamma) \mu_0$ with the relaxed inequality constraint $X^\top (K_\mathcal{D} w - (1-\gamma)\mu_0) \leq \epsilon_x$.
One applicable choice of the coefficient matrix $X$ would be a matrix that contains all $2^{|S|}$ binary (sign) vectors $[\pm 1, \pm 1, \ldots, \pm 1]$ in its columns.
Then, the inequality constraint is equivalent to the $\mathcal{L}^1$ norm constraint, i.e. $\Vert K_\mathcal{D} w - (1-\gamma)\mu_0 \Vert_1 \leq \epsilon_x$.

With this relaxation, the empirical version of the dual LP can be expressed as
\begin{equation}\label{eq:dual_offline}
\begin{split}
\max_{w \in \mathbb{R}^{|S||A|} } \quad &   u_\mathcal{D}^\top w \\
\text{s.t.} \quad & X^\top (K_\mathcal{D} w - (1-\gamma)\mu_0) \leq \epsilon_x, \quad w \geq 0.
\end{split}
\end{equation}
Additionally, the dual of \eqref{eq:dual_offline} can be expressed as
\begin{equation}\label{eq:primal_offline}
\begin{split}
\min_{v \in \mathbb{R}^{N_x}} \quad &   (1-\gamma)\mu_0^\top X v + \epsilon_x^\top v\\
\text{s.t.} \quad & K_\mathcal{D}^\top X v \geq u_\mathcal{D}, \quad v \geq 0,
\end{split}
\end{equation}
where $v$ is an optimization variable.

\paragraph{Feasible reward set estimation.}
Under the empirical LP formulations, our goal is to estimate the set of $u$ such that $w_e$ is (near) optimal to~\eqref{eq:dual_offline}.
Consider the primal-dual optimality conditions of $(v, w)$ under a reward function $u$:
\begin{equation}\label{eq:kkt}
\begin{split}
    &\text{(Primal feasibility)}: K_\mathcal{D}^\top X v \geq u, \; v \geq 0,\\
    &\text{(Dual feasibility)}: X^\top (K_\mathcal{D} w - (1-\gamma)\mu_0) \leq \epsilon_x, \; w \geq 0,\\
    &\text{(Zero duality gap)}: (1-\gamma)\mu_0^\top X v + \epsilon_x^\top v = u^\top w.
\end{split}
\end{equation}
$w$ is dual-optimal under $u$ if and only if the above optimality conditions hold with some $v$. 

Consequently, the feasible reward set can be estimated by identifying $(u, v)$ pairs for which $(u, v, w_e)$ satisfies \eqref{eq:kkt}.
Here, we further relax the zero duality gap condition with the slack parameter $\epsilon_g \geq 0$ for two reasons. First, the true reward might not satisfy this equality constraint due to errors in empirical estimation of $d_e$ and $K$.
Second, we are also interested in the reward such that $\pi_e$ is near-optimal.
Therefore, we consider the following polyhedron as an estimate of the feasible reward set:
\begin{equation}\label{eq:solution}
\hat{\mathcal{R}}_\text{IRL}(\epsilon_g) :=  \{(u, v) \mid \underbrace{(1-\gamma)\mu_0^\top X v + \epsilon_x^\top v   -  u^\top \mathbf{1} \leq \epsilon_g}_{(i)},\; \underbrace{K_\mathcal{D}^\top X v \geq u, \; v \geq 0}_{(ii)}, \; \underbrace{ -\hat{d}_e \leq u \leq \hat{d}_e}_{(iii)} \}.
\end{equation}
The constraint $(i)$ denotes the upper bound on the duality gap, where $\epsilon_g$ is used as the parameter.
$(ii)$ represents primal feasibility condition and $(iii)$ bounds the reward $r$ to the range $[-1, 1]$.
The vector $\mathbf{1}$ (vector of all ones) is used instead of $w_e$ in $(i)$, since $u^\top \mathbf{1} = u^\top w_e$ holds by the definition of $u$ and $w_e$.
Note that the dual feasibility condition is not required in $\hat{\mathcal{R}}_\text{IRL}(\epsilon_g)$ because it is a condition for the constant value $w_e$.



\subsection{Optimality Guarantee for Offline IRL}\label{sec:IRLoptimality}
In this section, we analyze the statistical error involved in the estimate $\hat{\mathcal{R}}_\text{IRL}$ of the feasible reward set $\mathcal{R}$.
Before presenting the main results, we address the data coverage issue in our setting.
In offline RL, distribution mismatch between the target policy and the behavior policy causes the inaccurate policy evaluation, and the concentrability-type assumption is required for an optimality guarantee.
In offline IRL, since the behavior policy is identical to the expert policy, the reward estimation can be inaccurate for state-actions pairs where the occupancy measure $d_e(s,a)$ is small.
We address this issue by defining the confident set of occupancy measures.

\paragraph{Confidence set.}
The confidence set if defined as the intersection of a set of valid occupancy measure (under MDP $\mathcal{M}$) and an $\mathcal{L}^\infty$ norm ball with radius $B$:
\begin{equation}
D_B :=  \left\{ d \in \mathbb{R}_+^{|S||A|} \mid M d = (1-\gamma)\mu_0, \; \Vert w_d \Vert_\infty \leq B \right\}.
\end{equation}
The radius $B\geq1$ is a parameter that controls the conservativeness of the algorithm. 

The set $D_B$ includes all possible occupancy measures $d$ if $B \geq d_\text{min}^{-1}$, where
\begin{equation}
d_\text{min} := \min_{(s,a) \in S \times A:\;d_e(s,a) \neq 0}d_e(s,a),    
\end{equation}
since $w_d(s,a) \leq d_\text{min}^{-1}$ for any $d \in \Delta(S\times A)$ and $(s,a) \in S \times A$ by the definition of $w_d$~\eqref{eq:w}.
In this case, optimality over the set $D_B$ implies global optimality.


It is worth highlighting that setting $B = d_\text{min}^{-1}$ yields results comparable to those in recent works~\cite{metelli2023towards, zhao2023inverse}.
The error bounds in these works depend on the constant $\pi_\text{min}^{-1}$, defined as
\begin{equation}
\pi_\text{min} := \min_{(s,a) \in S \times A:\;\pi_e(a | s) \neq 0} \pi_e(a | s).
\end{equation}
Under a fixed $\mu_0$, the value of $B = d_\text{min}^{-1}$ is upper bounded by $(\text{constant}) \times \pi_\text{min}^{-1}$, by the following inequality:
\begin{equation}
    d_\text{min} = d_e (s',a') = \pi_e(a' | s') \sum_{a \in A} d_e (s',a) \geq (1 -\gamma) \mu_0(s') \pi_\text{min},    
\end{equation}
where $(s', a') \in S \times A$ is a state-action pair that achieves the minimum in $d_\text{min}$.
Thus, setting $B = d_\text{min}^{-1}$ can provide error bounds comparable to those in other works while ensuring global optimality.


Our goal is to establish the optimality of $d_e$ within the confidence set $D_B$.
The proof comprises two distinct steps.
Firstly, we establish that $w_{\tilde{d}}$ is feasible to the dual empirical LP~\eqref{eq:dual_offline} with high probability for any $\tilde{d} \in D_B$, under appropriate level of relaxation $\epsilon_x$.
Next, we show that $w_e$ has a (nearly) higher objective than $w_{\tilde{d}}$ with high probability since $w_e$ has a small duality gap.
In the following lemma, we prove that for any $\tilde{d} \in D_B$, corresponding $w_{\tilde{d}}$ is a feasible solution to the empirical LP with high probability under appropriate relaxation level $\epsilon_x$ in the constraint.
\begin{lemma}\label{lem:feasibility}
In dual empirical LP~\eqref{eq:dual_offline}, let 
\begin{equation}
    \epsilon_x =  \Bigg(B(1+\gamma)\gamma^H  + B(1+\gamma)(1-\gamma^H) \sqrt{\frac{2|S||A|}{N}\log \frac{2N_x}{\delta}}\Bigg) \mathbf{1},    
\end{equation}
where $\delta>0$. Then, for any $\tilde{d} \in D_B$, $w_{\tilde{d}}$ is feasible to~\eqref{eq:dual_offline} with probability at least $1 - \frac{\delta}{2^{|S||A|}}$.
\end{lemma}
\begin{proof}
See Appendix~\ref{app:lem:feasibility}.
\end{proof}

From the above Lemma, we establish the optimality guarantee in the following theorem.
Specifically, in words, under the reward function $r$ recovered from the set \eqref{eq:solution}, we show that $d_e$ is an $\tilde{O}(\sqrt{|S||A|/N})$-suboptimal solution over the confidence set $D_B$ with high probability.

\begin{theorem}\label{thm:optimality}
Suppose $(u_\mathcal{D}, v_\mathcal{D}) \in \hat{\mathcal{R}}_\text{IRL}(\epsilon_g)$, with the relaxation level $\epsilon_x$ specified in Lemma~\ref{lem:feasibility}.
Let $r$ satisfy
\begin{equation}
r(s,a) = \frac{u_\mathcal{D}(s,a)}{\hat{d}_e(s,a)}
\end{equation}
for all $(s, a) \in S \times A$, following the convention $0/0=0$. Then, we have
\begin{equation}
   \mathbb{P} (r^\top d_e \geq r^\top \tilde{d} - \epsilon, \;\; \forall \tilde{d} \in D_B) \geq 1 - 3 \delta,
\end{equation}
where 
\begin{equation}
    \epsilon = \epsilon_g + (1+B) \gamma^H + (1-\gamma^H)\sqrt{\frac{2}{N} \log \frac{1}{\delta}} +  B (1-\gamma^H)\sqrt{\frac{2|S||A|}{N} \log \frac{2}{\delta}}.    
\end{equation}
\end{theorem}
\begin{proof}
See Appendix~\ref{app:thm:optimality}.
\end{proof}

\paragraph{Sample complexity analysis.}
The proposed solution set achieves the $\tilde{O}(B(1-\gamma^H)\sqrt{|S||A|/N})$ sample complexity bound with additional error terms $\epsilon_g$ and $(1+B)\gamma^H$.
Note that the parameter $\epsilon_g$ can be set to $\epsilon_g = \tilde{O}(1/\sqrt{N})$ to match the sample complexity.
The term $(1+B)\gamma^H$ diminishes exponentially with the horizon of the collected trajectory data, which underscores the requirement for long-horizon data to ensure accurate estimation.
To the best of our knowledge, besides our work, \cite{zeng2023understanding} is the only other study that offers an optimality guarantee for the offline IRL problem under a discounted MDP, with a sample complexity of $\tilde{O}(1/\sqrt{N})$.
However, as their algorithm is based on a bi-level optimization approach and their error bound is given for the log-likelihood function, a direct comparison of their result with ours is not feasible.
The concurrent work by~\cite{zhao2023inverse} presents a comparable sample complexity for an episodic MDP. We provide a detailed comparison in Appendix~\ref{app:comparison}.


\paragraph{Trade-off between optimality and feasibility.}
In our formulation, there exists a trade-off between the optimality of the policy and the feasibility of the reward function, which is modulated by the parameter $\epsilon_g$.
The duality gap bound, denoted as $\epsilon_g$, adjusts the size of the solution set $\hat{\mathcal{R}}_\text{IRL}(\epsilon_g)$; this set expands with an increase in $\epsilon_g$.
$\epsilon_g$ can be reduced to $0$ without causing infeasibility, as the set $\hat{\mathcal{R}}_\text{IRL}(\epsilon_g)$ is always non-empty due to the trivial solution $(u, v) = (0, 0)$.
A smaller value of $\epsilon_g$ enhances the optimality of the expert policy $\pi_e$, as stated in Theorem~\ref{thm:optimality}.
However, excessively reducing $\epsilon_g$ can lead to overly greedy choices, resulting in trivial or degenerate solutions.
The impact of varying $\epsilon_g$ is demonstrated through numerical experiments in Section~\ref{sec:experiment}.


\paragraph{Function approximation.}
The proposed LP formulation is well-suited for function approximation (parameterization), which allows us to reduce both the computational cost and the size (dimension) of the solution set.
Consider the parameterization of the variable $(u, v)$ as $(u_\theta, v_\theta)$, where $\theta$ represents a parameter within the parameter space $\Theta \subset \mathbb{R}^k$, which we aim to explore.
If there exists a $\theta \in \Theta$ such that $(u_\theta, v_\theta) \in \hat{\mathcal{R}}_\text{IRL}(\epsilon_g)$, then the optimality guarantee provided in Theorem~\ref{thm:optimality} is preserved for the reward function recovered from $u_\theta$, while the computational complexity of the LP can be reduced to a polynomial in $k$, down from $|S||A|$.
It is important to note that this formulation remains a linear (or convex) program under linear (or convex) parameterization.
If non-convex function approximation is employed for high-dimensional or continuous state-action spaces, an efficient algorithm for solving the proposed optimization may be required; however, such an extension is beyond the scope of this work, and we defer this to future research.


\subsection{Degeneracy Issue in Reward Learning}\label{sec:IRLdegeneracy}
In the practical applications of reward learning, estimating the feasible reward set is not enough; we need to select a single reward function within the estimated feasible reward set to use.
This is not a trivial problem due to existence of degenerate reward functions in the feasible reward set.
Degenerate reward functions (e.g. $r=\mathbf{0}$), though theoretically feasible, are practically undesirable as they fail to separate the expert policy $\pi_e$ from others.
In our solution set $\hat{\mathcal{R}}_\text{IRL}(\epsilon_g)$~\eqref{eq:solution}, degeneracy in the feasibility constraint $K_\mathcal{D}^\top X v \geq u$ is critical.
If equality holds for some state-action pairs such that $(K_\mathcal{D}^\top X v - u)(s, a) = 0$, then the complementary slackness condition will not be violated by changing the value of $w_e(s,a)$, meaning that $w_e$ may not be uniquely optimal. 
We suggest a simple and tractable method to obtain a non-degenerate reward function in $\hat{\mathcal{R}}_\text{IRL}(\epsilon_g)$.


\paragraph{Utilizing suboptimal trajectory samples.}
A straightforward approach to obtain a non-degenerate solution is utilizing a suboptimal policy $\pi_\text{sub}$.
To be specific, we directly maximize the expected reward gap between the expert policy $\pi_e$ and the suboptimal $\pi_\text{sub}$.
A viable example of $\pi_\text{sub}$ is a uniformly random policy such as $\pi_\text{sub}(a|s) = \frac{1}{|A|}$ $\forall (s,a) \in S \times A$, because this policy is unlikely to be optimal unless the expected rewards are uniform over all actions.
To maximize the reward gap, we sample suboptimal trajectories with $\pi_\text{sub}$ and estimate the occupancy measure of $\pi_\text{sub}$ as $\hat{d}_\text{sub}$, using the sampling and estimation methods discussed previously. 
Then, we maximize the empirical mean of the reward gap as per the following LP:
\begin{equation}\label{eq:irl}
\begin{split}
\max_{r ,u, v} \quad &  r^\top  (\hat{d}_e -\hat{d}_\text{sub}) \\
\text{s.t.} \quad & (u, v) \in \hat{\mathcal{R}}_\text{IRL}(\epsilon_g), \quad u = \hat{d}_e \circ r.
\end{split}
\end{equation}
Here, $\circ$ denotes the element-wise (Hadamard) product.
The numerical experiments in Section~\ref{sec:experiment} demonstrate that the above formulation efficiently recovers a non-degenerate reward function with only a small number of suboptimal trajectory samples.

%[[We can show that for suitable $\epsilon_g$, the underline $r$ should be within the set we obtained.]]

==> sections/section4_arXiv.tex <==
\section{Offline Reinforcement Learning from Human Feedback}
\subsection{LP Formulation of Offline RLHF}\label{sec:RLHFformulation}
In this section, we extend our LP framework to address offline RLHF problem.
As discussed in Section~\ref{sec:formulation:feedback}, our focus is on minimizing the error associated with the reward $r$ and the human feedback data $\mathcal{D}_\text{HF}$.
We begin by representing the cumulative reward of each trajectory $\tau^{n, i}$ ($i=1, 2$) in the dataset $\mathcal{D}_\text{HF}$ as a linear function of the reward $r$.
Specifically, the cumulative reward from the trajectory $\tau^{n, i}$ can be expressed as $r(\tau^{n, i}) = r^\top \psi^{n, i}$, where each vector $\psi^{n, i} \in \mathbb{R}^{|S||A|}$ can be mapped from the trajectory $\tau^{n, i}$ by
\begin{equation}\label{eq:vectorization}
    \psi^{n,i} (s, a) :=  \sum_{h=0}^{H-1} \gamma^h \mathbf{1}_{\{s_h^{n, i} = s, a_h^{n, i} = a\}},
\end{equation}
for any $(s,a) \in S \times A$.
Following this, we define the error in the single data point $(\tau^{n, 1},  \tau^{n, 2}, y^n)$ associated with the reward function $r$ as
\begin{equation}
\mathcal{L} (\tau^{n, 1},  \tau^{n, 2}, y^n ; r) :=  r^\top (\psi^{n, 2} - \psi^{n, 1}) \mathbf{1}_{\{y^n = 1\}}  + r^\top (\psi^{n, 1} - \psi^{n, 2}) \mathbf{1}_{\{y^n = 2\}}.    
\end{equation}

Note that naively minimizing the average or maximum error over queries might often lead to degenerate reward functions. 
This is because human evaluators sometimes provide conflicting feedback, such as $y^n=1$ when $r^\top \psi^{n, 2} > r^\top \psi^{n, 1}$, due to their stochasticity.
Under conflicting comparison data, minimizing $\mathcal{L}$ may result in degenerate solutions such as $r=\mathbf{0}$.
To address this issue, we allows for a slack in the error $\mathcal{L}$ by introducing a parameter $\epsilon_r \in \mathbb{R}$, which controls the size of the solution set.
Specifically, we define the solution set $\hat{\mathcal{R}}_\text{HF}$ as follows:
\begin{equation}\label{eq:RLHFset}
    \hat{\mathcal{R}}_\text{HF}(\epsilon_r) :=  \{r \mid  \mathcal{L} (\tau^{n, 1},  \tau^{n, 2}, y^n ; r)  \leq \epsilon_r \; \forall n=1, 2, \ldots, N_q, \quad  r\in [-1, 1]^{|S||A|}\}.    
\end{equation}
Under this adjustable solution set, if we have additional information, we could also apply the strategy discussed in the previous section for identifying non-degenerate solutions: maximizing the reward gap between the expert trajectories and the suboptimal trajectories.

One advantage of the proposed LP method is its robustness to different human evaluator preference models, in contrast to MLE-based algorithms.
When the human evaluator deviates from the preference model assumed in MLE, the true reward parameter may diverge from the parameter space.
However, the LP approach is not subject to this limitation.
We illustrate this point with a bandit example in Appendix~\ref{app:mle}, where our LP algorithm successfully finds an optimal policy, whereas the recent pessimistic MLE algorithm fail to do so.


\subsection{Generalization Guarantee for Offline RLHF}
Recent works in offline RLHF, such as \cite{zhu2023principled, zhan2023provable}, have proposed a pessimistic MLE algorithm and provided an error bound between the estimated and the true reward function of the supposed preference model.
Our LP method does not offer an optimality guarantee in the same way as these works, as it obtains a set of reward functions without assuming a specific preference model.
Instead, we analyze the generalization property of the obtained reward functions by examining how $r \in \hat{\mathcal{R}}_\text{HF}(\epsilon_r)$ aligns with unseen trajectory pairs sampled from $\mu_\text{HF}$.


We first introduce the probabilistic preference model for a human evaluator generating feedback data.
We emphasize that our proposed method is not dependent on this model; we introduce it to analyze a generalization property.
Suppose that $y \in \{1, 2\}$ is sampled from a Bernoulli distribution with the probabilistic model $\mathbb{P}(y = 1 \mid \tau^{1}, \tau^{2}) = \Phi(r_\text{true}^\top (\psi^{1} - \psi^{2}))$, where $\Phi:\mathbb{R} \mapsto [0, 1]$ is a  monotonically non-decreasing function satisfying $\Phi(x) + \Phi(-x) = 1$ for all $x \in \mathbb{R}$. 
$\Phi$ represents the preference model of the evaluator, based on their personal reward function $r_\text{true}$.
For example, if $\Phi$ is a sigmoid function, i.e. $\Phi(x) = 1/(1+e^{-x})$, then the above probabilistic model is reduced to the Bradley-Terry-Luce (BTL) model~\cite{christiano2017deep}.
In the following theorem, we provide a generalization guarantee of any reward functions $r$ contained in the estimated solution set $\hat{\mathcal{R}}_\text{HF}(\epsilon_r)$.
Specifically, for a random (unseen) trajectory pair $(\tau^1, \tau^2)$ sampled from the sampling distribution $\mu_\text{HF}$ and the human feedback $y$ sampled from the preference model $\Phi$, we prove that the error $\mathcal{L} ( \tau^{1},  \tau^{2}, y; r)$ is bounded by $\epsilon_r$ with high probability.


\begin{theorem}\label{thm:rlhf}
Suppose $r \in \hat{\mathcal{R}}_{\text{HF}}(\epsilon_r)$ and the human feedback data $(\tau^1, \tau^2, y) $ is sampled i.i.d. from the joint distribution $(\mu_{\text{HF}}, \Phi)$.
Then, for any $\delta \in (0, 1)$, 
\begin{equation}
     \mathbb{P} \left( \mathcal{L} ( \tau^{1},  \tau^{2}, y; r) \geq \epsilon_r \right) \leq \sqrt{\frac{1}{2 N_q} \log \frac{1}{\delta}}
\end{equation}
holds with probability at least $ 1-\delta $.
\end{theorem}
\begin{proof}
See Appendix~\ref{app:thm:rlhf}.
\end{proof}

Note that a trade-off between optimality and feasibility exists in $\hat{\mathcal{R}}_{\text{HF}}(\epsilon_r)$ with respect to the parameter $\epsilon_r$, similar to $\hat{\mathcal{R}}_{\text{IRL}}(\epsilon_g)$ in offline IRL.
Specifically, while it is preferable to set the parameter $\epsilon_r$ as small as possible to avoid overly relaxing the RLHF constraint, excessively reducing $\epsilon_r$ can lead to feasibility issues.
In practice, if any prior knowledge about the preference model $\Phi$ is available, this information can guide the selection of $\epsilon_r$.
If no such information is available, $\epsilon_r$ can be determined experimentally by starting with a large value and gradually reducing it until the reward set becomes trivial or infeasible.





\subsection{Integration of IRL and RLHF}\label{sec:integration}
Finally, our LP framework facilitates the integration of two types of expert data: IRL (trajectories collected from the expert policy) and RLHF (pairwise trajectory comparisons).
This is a unique feature of our LP framework, one that remains unexplored in the MLE framework.
We propose to recover the reward function $r$ from the intersection of two sets $\hat{\mathcal{R}}_\text{IRL}(\epsilon_g)$ and $\hat{\mathcal{R}}_\text{HF}(\epsilon_r)$ such that
\begin{equation}\label{eq:irl-rlhf:d}
\hat{\mathcal{R}}_\text{IRL-HF}(\epsilon_g, \epsilon_r) = \{ (r, u, v) \mid (u, v) \in \hat{\mathcal{R}}_\text{IRL}(\epsilon_g),\; r \in \hat{\mathcal{R}}_\text{HF}(\epsilon_r), \; u = \hat{d}_e \circ r\}.
\end{equation}
In this combined formulation, the IRL constraint $(u, v) \in \hat{\mathcal{R}}_\text{IRL}(\epsilon_g)$ provides the optimality guarantee of the expert policy, while the RLHF constraint $r \in \hat{\mathcal{R}}_\text{HF}(\epsilon_r)$ reduces the solution set and mitigates degeneracy by imposing additional constraints.

\paragraph{Strict trajectory comparison.}
If we can impose a strict reward gap between two trajectories, then the RLHF constraint can mitigate degeneracy more effectively.
For instance, the constraint $r(\tau^1) \geq r(\tau^2) + \delta$ eliminates degenerate solutions that satisfy $r(\tau^1) = r(\tau^2)$ from the solution set, if we can set a strict reward gap $\delta > 0$ based on human feedback data.
To formalize this, we extend our approach to include the continuous feedback case, wherein the feedback is given as a continuous variable, $y \in [-1, 1]$, instead of the discrete variable used in previous sections.
In Appendix~\ref{app:continuous}, we specify this continuous feedback setting, and suggest how we can extend the definition of the solution set $\hat{\mathcal{R}}_\text{HF}(\epsilon_r)$ as well as the generalization guarantee provided in Theorem~\ref{thm:rlhf}.
Additionally, in the next section, we compare the effects of discrete and continuous human feedback through numerical experiments.




